TEaR: Improving LLM-based Machine Translation with Systematic Self-Refinement

Large Language Models (LLMs) have achieved impressive results in Machine Translation (MT). However, careful evaluations by human reveal that the translations produced by LLMs still contain multiple errors. Importantly, feeding back such error information into the LLMs can lead to self-refinement and result in improved translation performance. Motivated by these insights, we introduce a systematic LLM-based self-refinement translation framework, named \textbf{TEaR}, which stands for \textbf{T}ranslate, \textbf{E}stimate, \textbf{a}nd \textbf{R}efine, marking a significant step forward in this direction. Our findings demonstrate that 1) our self-refinement framework successfully assists LLMs in improving their translation quality across a wide range of languages, whether it's from high-resource languages to low-resource ones or whether it's English-centric or centered around other languages; 2) TEaR exhibits superior systematicity and interpretability; 3) different estimation strategies yield varied impacts, directly affecting the effectiveness of the final corrections. Additionally, traditional neural translation models and evaluation models operate separately, often focusing on singular tasks due to their limited capabilities, while general-purpose LLMs possess the capability to undertake both tasks simultaneously. We further conduct cross-model correction experiments to investigate the potential relationship between the translation and evaluation capabilities of general-purpose LLMs. Our code and data are available at https://github.com/fzp0424/self_correct_mt

==> Tables/all_stat.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table*}
\centering
% \vskip 0.15in
\resizebox{\textwidth}{!}{%
\begin{tabular}{cclccclccc} 
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Language Pair}} & \multirow{2}{*}{\textbf{Domain types}}  & \multicolumn{3}{c}{\textbf{General Machine Translation}}                                                                                                                   &  & \multicolumn{3}{c}{\textbf{Metrics Shared Task}}                         \\ 
\cmidrule{4-6}\cmidrule{8-10}
                                  &                                         &                                         & \multicolumn{1}{l}{\textbf{\textbf{Total Segments}}} & \multicolumn{1}{l}{\textbf{\textbf{Sampled Segments}}} & \multicolumn{1}{l}{\textbf{\textbf{\#tokens per segment}}} &  & \textbf{Selected Segments} & \textbf{Systems} & \textbf{Total Segments}  \\ 
\midrule
WMT22                             & En-Ru                                   & News, E-commerce                        & 2016                                                 & 200                                                    & 16.38                                                      &  & 59                         & 15               & 885                      \\ 
\midrule
WMT23                             & En-De                                   & Social, News, Meeting notes, E-commerce & 557                                                  & 200                                                    & 59.46                                                      &  & 80                         & 12               & 960                      \\
WMT23                             & He-En                                   & Social, News                            & 1910                                                 & 200                                                    & 21.66                                                      &  & 80                         & 12               & 960                      \\
WMT23                             & Zh-En                                   & Manuals, News, E-commerce               & 1976                                                 & 200                                                    & 22.85                                                      &  & 80                         & 15               & 1200                     \\
\bottomrule
\end{tabular}
}
\caption{Statistics of our testset. \textit{\#tokens per segment} indicates the average number of tokens of the translation pairs, calculated based on the sampled text from the English portion of either the source or reference. \textit{Systems}: translation systems that are annotated in the WMT for the given year.}
\label{all:stat}
% \vskip -0.1in
\end{table*}

==> Tables/app_module.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table*}
\centering
\caption{The results of testing translation ability of various LLMs under 5-shot setting in our sampled WMT23 datasets.}
\vskip 0.15in
\label{tab:app_module}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccccccccc} 
\toprule
\multicolumn{2}{c}{\textbf{Translate }} &  & \multicolumn{2}{c}{\textbf{Estimate }} &  & \multicolumn{2}{c}{\textbf{Refine }}   &  & \multirow{2}{*}{\textbf{\# of tested}} & \multirow{2}{*}{} & \multirow{2}{*}{\textbf{BLEU}} &  & \multirow{2}{*}{\textbf{COMET}} &  & \multirow{2}{*}{\textbf{COMETKiwi}} &  & \multirow{2}{*}{\textbf{BLEURT}}  \\ 
\cmidrule{1-2}\cmidrule{4-5}\cmidrule{7-8}
\textbf{0-shot} & \textbf{5-shot}       &  & \textbf{0-shot} & \textbf{3-shot}      &  & \textbf{wo 5-shot} & \textbf{w 5-shot} &  &                                        &                   &                                &  &                                 &  &                                     &  &                                   \\ 
\midrule
\checkmark             &                       &  & -               & -                    &  & -                  & -                 &  & \multirow{10}{*}{200}                  &                   & 25.45                          &  & 80.01                           &  & 78.87                               &  & 66.56                             \\
\checkmark             &                       &  & \checkmark             &                      &  & \checkmark                &                   &  &                                        &                   & 24.95                          &  & 80.05                           &  & 78.95                               &  & 66.64                             \\
\checkmark             &                       &  & \checkmark             &                      &  &                    & \checkmark               &  &                                        &                   & 25.15                          &  & 80.22                           &  & 79.18                               &  & 66.91                             \\
\checkmark             &                       &  &                 & \checkmark                  &  & \checkmark                &                   &  &                                        &                   & 25.56                          &  & 80.52                           &  & 79.75                               &  & 67.01                             \\
\checkmark             &                       &  &                 & \checkmark                  &  &                    & \checkmark               &  &                                        &                   & 25.79                          &  & 80.68                           &  & 79.77                               &  & 67.09                             \\
                & \checkmark                   &  & -               & -                    &  & -                  & -                 &  &                                        &                   & 26.30                          &  & 80.31                           &  & 79.28                               &  & 67.07                             \\
                & \checkmark                   &  & \checkmark             &                      &  & \checkmark                &                   &  &                                        &                   & 26.12                          &  & 80.44                           &  & 79.71                               &  & 67.24                             \\
                & \checkmark                   &  & \checkmark             &                      &  &                    & \checkmark               &  &                                        &                   & 26.23                          &  & 80.54                           &  & 79.94                               &  & 67.33                             \\
                & \checkmark                   &  &                 & \checkmark                  &  & \checkmark                &                   &  &                                        &                   & 26.01                          &  & 80.52                           &  & 79.79                               &  & 67.66                             \\
                & \checkmark                   &  &                 & \checkmark                  &  &                    & \checkmark               &  &                                        &                   & \textbf{26.41}                 &  & \textbf{80.70}                  &  & \textbf{\textbf{80.07}}             &  & \textbf{\textbf{67.84}}           \\
\bottomrule
\end{tabular}
}
\vskip -0.1in
\end{table*}

==> Tables/cmp_estimate.tex <==
% \usepackage{booktabs}


\begin{table}
\centering
% \vskip 0.15in
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccc} 
\toprule
\multicolumn{1}{c}{\textbf{Estimation Method}} &                      & \textbf{BLEU} &                      & \textbf{COMET} &                      & \textbf{COMETKiwi} &                      & \textbf{BLEURT}  \\ 
\midrule
-                                              &                      & 24.70                      &                      & 78.67                       &                      & 77.22                           &                      & 64.28                         \\
\midrule
3-shot~                                        &                      & 24.36                  &                      & 79.50                   &                      & 78.91                      &                      & 65.91                     \\
Multi-step~                                    & \multicolumn{1}{l}{} & 23.89                  & \multicolumn{1}{l}{} & 79.72                    & \multicolumn{1}{l}{} & 78.59                        & \multicolumn{1}{l}{} & 65.83                     \\
GPT-4 w/ human                                 & \multicolumn{1}{l}{} & 29.25                   & \multicolumn{1}{l}{} & 81.19                   & \multicolumn{1}{l}{} & 78.85                       & \multicolumn{1}{l}{} & 69.08                      \\
\bottomrule
\end{tabular}
}
% \vskip -0.1in
\caption{Performance for different strategies in \textbf{Estimate} module. \textbf{Translate} module and \textbf{Refine} module are under the same settings. $''$-$''$ represents no estimation. \textit{w/ human} denotes with manual checking.}
\label{tab:cmp_estimate}
\end{table}

==> Tables/module.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table*}
\centering
% \vskip 0.15in
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccccccccccccc} 
\toprule
\multicolumn{2}{c}{\textbf{Translate }} &  & \multicolumn{2}{c}{\textbf{Estimate }} &  & \multicolumn{2}{c}{\textbf{Refine }}   &  & \multirow{2}{*}{\textbf{\# of refinements }} & \multirow{2}{*}{} & \multicolumn{2}{c}{\textbf{BLEU}} &  & \multicolumn{2}{c}{\textbf{COMET}} &  & \multicolumn{2}{c}{\textbf{COMETKiwi}} &  & \multicolumn{2}{c}{\textbf{BLEURT}}  \\ 
\cmidrule{1-2}\cmidrule{4-5}\cmidrule{7-8}\cmidrule{12-22}
\textbf{0-shot} & \textbf{5-shot}       &  & \textbf{0-shot} & \textbf{3-shot}      &  & \textbf{$\mathcal{T}_{refine}-\alpha$} & \textbf{$\mathcal{T}_{refine}-\beta$} &  &                                              &                   & \textbf{score} & \textbf{$\Delta$}       &  & \textbf{score} & \textbf{$\Delta$}        &  & \textbf{score} & \textbf{$\Delta$}            &  & \textbf{score} & \textbf{$\Delta$}          \\ 
\midrule
\checkmark              &                       &  & \checkmark              &                      &  & -                  & -                 &  & \multirow{3}{*}{123}                         &                   & 25.51          & -                &  & 79.78          & -                 &  & 78.85          & -                     &  & 65.84          & -                   \\
\checkmark              &                       &  & \checkmark              &                      &  & \checkmark                 &                   &  &                                              &                   & 24.29          & -1.22            &  & 79.85          & 0.07              &  & 78.98          & 0.13                  &  & 65.98          & 0.14                \\
\checkmark              &                       &  & \checkmark              &                      &  &                    & \checkmark                &  &                                              &                   & 24.54          & -0.97            &  & 80.12          & 0.34              &  & 79.35          & 0.50                  &  & 66.42          & 0.58                \\ 
\midrule
\checkmark              &                       &  &                 & \checkmark                   &  & -                  & -                 &  & \multirow{3}{*}{99}                          &                   & 24.24          & -                &  & 78.97          & -                 &  & 76.93          & -                     &  & 65.86          & -                   \\
\checkmark              &                       &  &                 & \checkmark                   &  & \checkmark                 &                   &  &                                              &                   & 24.15          & -0.09            &  & 80.00          & 1.03              &  & 78.71          & 1.78                  &  & 66.77          & 0.91                \\
\checkmark              &                       &  &                 & \checkmark                   &  &                    & \checkmark                &  &                                              &                   & 24.60          & 0.36             &  & 80.32          & 1.35              &  & 78.75          & 1.82                  &  & 66.94          & 1.08                \\ 
\midrule
                & \checkmark                    &  & \checkmark              &                      &  & -                  & -                 &  & \multirow{3}{*}{160}                         &                   & 27.06          & -                &  & 80.07          & -                 &  & 79.17          & -                     &  & 66.75          & -                   \\
                & \checkmark                    &  & \checkmark              &                      &  & \checkmark                 &                   &  &                                              &                   & 26.59          & -0.47            &  & 80.23          & 0.16              &  & 79.72          & 0.55                  &  & 66.96          & 0.21                \\
                & \checkmark                    &  & \checkmark              &                      &  &                    & \checkmark                &  &                                              &                   & 26.71          & -0.35            &  & 80.35          & 0.28              &  & 80.01          & 0.84                  &  & 67.07          & 0.32                \\ 
\midrule
                & \checkmark                    &  &                 & \checkmark                   &  & -                  & -                 &  & \multirow{5}{*}{94}                          &                   & 24.70          & -                &  & 78.67          & -                 &  & 77.22          & -                     &  & 64.28          & -                   \\
                & \checkmark                    &  &                 & \checkmark                   &  & \checkmark                 &                   &  &                                              &                   & 23.66          & -1.04            &  & 79.12          & 0.45              &  & 78.33          & 1.11                  &  & 65.53          & 1.25                \\
                & \checkmark                    &  &                 & \checkmark                   &  &                    & \checkmark                &  &                                              &                   & 24.36          & -0.34            &  & 79.50          & 0.83              &  & 78.91          & 1.69                  &  & 65.91          & 1.63                \\
                
\bottomrule
\end{tabular}
}
% \vskip -0.1in
\caption{xxx}
\label{tab:module}
\end{table*}
